TITUS: the Tokai Intermediate Tank for the Unoscillated Spectrum

The TITUS, Tokai Intermediate Tank for Unoscillated Spectrum, detector, is a proposed Gd-doped Water Cherenkov tank with a magnetised muon range detector downstream. It is located at J-PARC at about 2 km from the neutrino target and it is proposed as a potential near detector for the Hyper-Kamiokande experiment. Assuming a beam power of 1.3 MW and 27.05 x 10^{21} protons-on-target the sensitivity to CP and mixing parameters achieved by Hyper-Kamiokande with TITUS as a near detector is presented. Also, the potential of the detector for cross sections and Standard Model parameter determination, supernova neutrino and dark matter are shown.

==> NetronMultiplicity.tex <==
{\it writers: Francesca, Teppei}

